Fine-grained Angular Contrastive Learning with Coarse Labels

Few-shot learning methods offer pre-training techniques optimized for easier later adaptation of the model to new classes (unseen during training) using one or a few examples. This adaptivity to unseen classes is especially important for many practical applications where the pre-trained label space cannot remain fixed for effective use and the model needs to be "specialized" to support new categories on the fly. One particularly interesting scenario, essentially overlooked by the few-shot literature, is Coarse-to-Fine Few-Shot (C2FS), where the training classes (e.g. animals) are of much `coarser granularity' than the target (test) classes (e.g. breeds). A very practical example of C2FS is when the target classes are sub-classes of the training classes. Intuitively, it is especially challenging as (both regular and few-shot) supervised pre-training tends to learn to ignore intra-class variability which is essential for separating sub-classes. In this paper, we introduce a novel 'Angular normalization' module that allows to effectively combine supervised and self-supervised contrastive pre-training to approach the proposed C2FS task, demonstrating significant gains in a broad study over multiple baselines and datasets. We hope that this work will help to pave the way for future research on this new, challenging, and very practical topic of C2FS classification.

==> files/backup.tex <==
\subsection{Problem Definition}
The problem-space we tackle is as follows: consider two distinct sets of classes: $\mathcal{Y}_{fine}\{y_{00},...,y_{0k_0} , y_{10},...,y_{1k_1},...,y_{C0},...y_{Ck_C}\}$, and $\mathcal{Y}_{coarse}=\{y_0,...,y_C\}, |\mathcal{Y}_{coarse}|=C+1$. An image has both a coarse label and a fine label. A hierarchy is defined in a unique manner such that $\forall i,img: coarse\_class(img)=y_i \Longleftrightarrow fine\_class(img)\in \{y_{i0},...,y_{ik_i}\}$.

Given a training set, consisting of tuples of images and coarse labels: $\mathcal{S}=\{(img,y_i)|y_i\in \mathcal{Y}_{coarse}\}$, train a model to achieve maximum classification accuracy on a test set consisting of fine labels: $\mathcal{T}=\{(img,y_{ij})|y_{ij}\in \mathcal{Y}_{fine}\}$.

\subsection{Architecture}
At its core, our method focuses on leveraging supervised learning for coarse classes and unsupervised learning for fine classes, with high synergy.

This architecture is described in figure [?]. Our module initializes with three components: two different FCN backbones with an MLP on top, which we denote as $\mathcal{B}_q, \mathcal{B}_k$, and a set of queues for each coarse class, $\{\mathcall{Q}_i | 0<=i<=C\}$. For each queue: $\mathcal{Q}_i\in\mathbb{R}^{d\times K}$ where $d$ is the output dimension of $\mathcal{B}_q$ and $\mathcal{B}_k$, and $K$ is a hyper-parameter determining the size of the queues. Like in \cite{HeMomentumLearning}, $\mathcal{B}_q$ is updated via back-propagation while $\mathcal{B}_k$ is updated via momentum relative to $\mathcal{B}_q$. Also similarly, the outputs of $\mathcal{B}_k$ are stored over time in a queue. However, unlike \cite{HeMomentumLearning}, we store these outputs in a $\mathcal{Q}_i$ of the corresponding coarse class, as opposed to storing all samples in the same queue.

Given an image $I$ of coarse class $y_i: i<=C$, we create two different augmentations $I_q,I_k$. Each augmentation is passed through the two backbones to retrieve  $q=\mathcal{B}_q(I_q), k_+=\mathcal{B}_k(I_k)$.

At this point, we compute two loss functions:

1. \textbf{Coarse Cross-Entropy Loss}: Given $q$, and the coarse label vector $y=(0,...,1,...,0): y_i=1$. We first use a linear classifier $W\in{\mathbb{R}^{d\times C}}$ to compute coarse class logits $l=W(q)$. Then, we calculate softmax and cross-entropy loss on $l$, which we denote $\mathcal{L}_{cls}(l,y)$.

2. \textbf{Fine Contrastive Loss}: Given $q$, $k_+$, and the set of stored embeddings in $\{k_0,...\} = \mathcal{Q}_i$, we first pass every embedding into the coarse class-normalization component $\mathcal{A}_i$, which we expand upon below, to retrieve the components $q_\angle=\mathcal{A}_i(q), k_{+_\angle}=\mathcal{A}_i(k_+)$, and $\{k_{0_\angle},...\}=\{\mathcal{A}_i(k_0),...\}$. Then, we calculate InfoNCE loss with the former pair serving as the positives, and the latter set as negatives. We denote this loss $\mathcal{L}_{cst}(q_\angle,k_{+_\angle},\{k_{0_\angle},...\})$.

Finally, our loss function is: 
\begin{equation}
\mathcal{L}=\mathcal{L}_{cls} + \mathcal{L}_{cst}    
\end{equation}


\subsection{Class-normalized Angular Contrast}
We present a novel approach that creates a synergy between the supervised and self-supervised loss components. First, we define a \textbf{coarse class-weight} for class $y_i$ as the $i_{th}$ column of $W$: $W_i\in \mathbb{R}^d$.

In regular contrastive learning, $q$ and any $k\in\mathca{Q}_i$
Given $q$ and any $k\in\mathcal{Q}_i$, a standard supervised classification component, will teach the network to push $q$ and  $k$ as close as possible to their corresponding class weight $w$. However, a conventional contrastive learning loss will teach the network to pull these two features apart. As can be seen in figure [?](a), the result of a naive combination of $\mathcal{L}_{cls}$ and $\mathcal{L}_{cst}$ will result in a conflict between them, since a by-product of pushing away samples from each-other is these samples being pushed away from $\mathcal{W}_i$. This results in sub-optimal training.

Our proposed solution which we term as Class-normalized Angular Contrast, is to alter the contrastive component: rather than having the loss optimize for maximal euclidean distance between samples of the same coarse class, it should optimize for maximal dispersion of samples \textit{within a specific coarse class}. Instead, our method is to find the angles between $q$ and $k$, with their class-weight $W_i$ as anchor. This way, our contrastive component doesn't push the samples away from $W_i$, but rather it pushes those samples \textit{around} it, as can be seen in figure [?](b). In this case, the coarse classification component of training is not harmed by the contrastive one, but our model still learns to distinguish between examples of the same coarse class, which gives it the ability to generalize well to fine classes.

In practice, this can be achieved by introducing a simple component prior to the calculation of $\mathcal{L}_{cst}$, which we denote as $\mathcal{A}_i$, which normalizes the value of its input relative to the class weight $W_i$. Formally, this is done by:
\begin{equation}
\mathcal{A}_i(v)=v_\angle=\frac{\frac{v_1}{\rVert{v_1}\rVert} - \frac{\mathcal{W}_i}{\rVert\mathcal{W}_i\rVert}}{\rVert\frac{v_1}{\rVert{v_1}\rVert} - \frac{\mathcal{W}_i}{\rVert\mathcal{W}_i\rVert}\rVert}
\end{equation}

As can be seen in figure [?](b), the dot product between two class-normalized embeddings $v,u$: $v\cdot u=\rVert v \rVert \cdot \rVert u \rVert \cdot cos\theta=cos\theta$. This means that in practice, the logits used in the infoNCE loss $\mathcal{L}_{cst}$ are cosines of angles, and the model will learn to optimize for these angles rather than plain distance.



% We study the performance of \oursspace further, to find in which domains it performs better than its counterparts. Specifically, we're interested in two questions:

% 1. Is the performance improvement we witness caused by being able to  distinguish between fine classes better, as we originally hypothesized, or was caused simply by being able to distinguish between the coarse classes better?

% 2. Why are the gaps in performance in the all-way task considerably bigger than those in the 5-way task?

% For this purpose, we introduce table \ref{tab:coarse_vs_fine}, which compares the performance of the baselines in two additional tasks: all-way 1-shot on coarse classes (FOOTNOTE: Using a metric method for coarse classification isn't a fair comparison
% relative to using the linear classifier with which the models have trained, but because this is in the context of fine classification, we're interested in the metric properties of our space without intense classifier training), 
% and \textit{fine 5-way 1-shot}, which is a few shot task where the five ways always sub-class the same coarse class.

% In this table, we can see the clearly-visible trade-off between coarse and fine performance. In the coarse task, The gaps in performance between \oursspace and the regular coarse model are small, but the gap in fine performance is significant. With the coarse (mlp) model, the exact opposite happens: The gap in coarse performance is great, while the gap in fine performance is significantly smaller. Thanks to angular contrast, our model benefits from improved performance in the fine domain, without suffering in the coarse domain, so we don't have to choose between the trade-offs.

% Finally, we can see that the all-way task on fine classes encapsulates both of the tasks above adequately, which is why we found it crucial to include it together with the commonly-used 5-way task.

% We hypothesize that the reasoning behind this is that a regular 5-way test, is more similar to a
% test on coarse classification performance rather than fine. Specifically on LIVING-17, the odds of sampling 5 samples by fine class, which don't even share a coarse class is 52\%. As such, distinguishing between the samples could 
% be as easy as distinguishing between coarse classes rather than fine classes.

% On the other hand, we see significantly bigger gaps in performance on the fine 5-way task, confirming our assertion that \oursspace improves fine-grained separability. Finally, we believe that the all-way fine classification task encapsulates
% both of the metrics noted above adequately, and is why we found it to be crucial to include it in the first place, as opposed to 5-way alone.

==> tables/coarse_classification.tex <==
\begin{table}[]
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
                       & living17              & nonliving26           & entity13              & entity30              \\ 
\midrule
\multicolumn{2}{l}{\textbf{Linear Classifier}}                                                     \\
Coarse                 & 93.74                 & 86.25                 & 87.54                 & 88.78                 \\
Coarse (mlp)           & \textbf{94.85}        & 87.73                 & 91.80                  & 89.51                 \\
Ours                   & 94.15                 & \textbf{88.08}        & \textbf{92.28}        & \textbf{89.83}        \\ 
\midrule
\multicolumn{2}{l}{\textbf{All-way Cosine NN}}                                                            \\
                    %   & living17              & nonliving26           & entity13              & entity30              \\ 
% \midrule
Coarse                 & 81.44 \scriptsize{$\pm$ 0.31}          & 60.56 \scriptsize{$\pm$ 0.29}          & 68.3 \scriptsize{$\pm$ 0.40}            & \textbf{69.18 \scriptsize{$\pm$ 0.27}} \\
Coarse (mlp)           & 50.83 \scriptsize{$\pm$ 0.32}          & 35.36 \scriptsize{$\pm$ 0.23}          & 41.07 \scriptsize{$\pm$ 0.35}          & 39.74 \scriptsize{$\pm$ 0.22}          \\
Ours                   & \textbf{84.25 \scriptsize{$\pm$ 0.31}} & \textbf{67.13 \scriptsize{$\pm$ 0.29}} & \textbf{72.19 \scriptsize{$\pm$ 0.39}} & 64.03 \scriptsize{$\pm$ 0.26}          \\ 
\bottomrule
\end{tabular}}
\captionof{table}{Coarse performance}
    \vspace{-10pt}
\label{tab:coarse}
\end{table}
